The equidistant dimension of some graphs of convex polytopes

This paper is devoted to some rotationally symmetric classes of graphs denoted in literature as convex polytope graphs. Exact value of equidistant dimension is found for $T_n$. Next, for even $n$ exact values are found for $R''_n$ and $S''_n$, while for odd $n$ exact value is found for $S_n$. Finally, for odd $n$, lower bound are found for $R''_n$ and $S''_n$.

==> an.tex <==
\begin{figure}[htbp]
    \centering\setlength\unitlength{1mm}

\setlength\unitlength{1mm}
\begin{picture}(130,35)
\thicklines
\tiny
\put(47.7,5.0){\circle*{1}} \put(47.7,5.0){\line(1,1){7.3}} \put(47.7,5.0){\line(-4,-1){9.7}} \put(47.7,5.0){\line(-1,4){2.5}} 
\put(55.0,12.3){\circle*{1}} \put(55.0,12.3){\line(4,1){10.0}} \put(55.0,12.3){\line(-4,1){9.8}} \put(55.0,12.3){\line(1,4){2.8}} 
\put(65.0,15.0){\circle*{1}} \put(65.0,15.0){\line(4,-1){10.0}} \put(65.0,15.0){\line(-1,1){7.2}} \put(65.0,15.0){\line(1,1){7.2}} 
\put(75.0,12.3){\circle*{1}} \put(75.0,12.3){\line(1,-1){7.3}} \put(75.0,12.3){\line(-1,4){2.8}} \put(75.0,12.3){\line(4,1){9.8}} 
\put(82.3,5.0){\circle*{1}} \put(82.3,5.0){\line(1,4){2.5}} \put(82.3,5.0){\line(4,-1){9.7}} 
\put(38.0,2.2){\circle*{1}} \put(38.0,2.2){\line(3,5){7.2}} \put(38.0,2.2){\line(0,1){19.6}} \put(38.0,2.2){\line(-4,1){9.7}} 
\put(45.2,14.8){\circle*{1}} \put(45.2,14.8){\line(5,3){12.6}} \put(45.2,14.8){\line(3,5){10.0}} \put(45.2,14.8){\line(-1,1){7.1}} 
\put(57.8,22.0){\circle*{1}} \put(57.8,22.0){\line(1,0){14.5}} \put(57.8,22.0){\line(5,3){17.1}} \put(57.8,22.0){\line(-1,4){2.6}} 
\put(72.2,22.0){\circle*{1}} \put(72.2,22.0){\line(5,-3){12.6}} \put(72.2,22.0){\line(1,0){19.6}} \put(72.2,22.0){\line(1,4){2.6}} 
\put(84.8,14.8){\circle*{1}} \put(84.8,14.8){\line(3,-5){7.2}} \put(84.8,14.8){\line(5,-3){16.9}} \put(84.8,14.8){\line(1,1){7.1}} 
\put(92.0,2.2){\circle*{1}} \put(92.0,2.2){\line(4,1){9.7}} 
\put(28.3,4.8){\circle*{1}} \put(28.3,4.8){\line(3,5){9.8}} 
\put(38.1,21.9){\circle*{1}} \put(38.1,21.9){\line(5,3){17.0}} 
\put(55.2,31.7){\circle*{1}} \put(55.2,31.7){\line(1,0){19.7}} 
\put(74.8,31.7){\circle*{1}} \put(74.8,31.7){\line(5,-3){17.0}} 
\put(91.9,21.9){\circle*{1}} \put(91.9,21.9){\line(3,-5){9.8}} 
\put(101.7,4.8){\circle*{1}}
\thinlines
\put(47.7,5.0){\line(-1,-2){2}} \put(82.3,5.0){\line(1,-2){2}}
\put(38.0,2.2){\line(1,-1){4}} \put(92.0,2.2){\line(-1,-1){4}}
\put(38.0,2.2){\line(0,-1){5}} \put(92.0,2.2){\line(0,-1){5}}
\put(28.3,4.8){\line(0,-1){5}} \put(101.7,4.8){\line(0,-1){5}}
\put(28.3,4.8){\line(1,-1){4}} \put(101.7,4.8){\line(-1,-1){4}}
\put(48.3,3.5){$a_2$} \put(54.5,9.7){$a_1$} \put(63.0,12.0){$a_0$} \put(71,9.7){$a_{n-1}$} \put(76.5,3.5){$a_{n-2}$} 
\put(34.5,0.5){$b_2$} \put(41.2,14.5){$b_1$} \put(54.0,23.3){$b_0$} \put(67.2,24.5){$b_{n-1}$} \put(81.6,17.8){$b_{n-2}$} \put(92.3,4.5){$b_{n-3}$} 
\put(25,5.4){$c_2$} \put(35.7,23.3){$c_1$} \put(53.6,33.6){$c_0$} \put(74.4,33.6){$c_{n-1}$} \put(92.3,23.3){$c_{n-2}$} \put(102.6,5.4){$c_{n-3}$} 

\end{picture}
    \caption{\label{fig:an} \small The graph of convex polytope $A_n$}
\end{figure}

